Excited $J^{--}$ meson resonances at the SU(3) flavor point from lattice QCD

We present the first calculation within lattice QCD of excited light meson resonances with $J^{PC} = 1^{--}$, $2^{--}$ and $3^{--}$. Working with an exact SU(3) flavor symmetry, for the singlet representation of pseudoscalar-vector scattering, we find two $1^{--}$ resonances, a lighter broad state and a heavier narrow state, a broad $2^{--}$ resonance decaying in both $P$- and $F$-waves, and a narrow $3^{--}$ state. We present connections to experimental $\omega^\star_J, \phi^\star_J$ resonances decaying into $\pi \rho$, $K\bar{K}^*$, $\eta \omega$ and other final states.

==> amps.tex <==
% !TEX root = ../paper.tex

The relationship between the $t$-matrix describing scattering and the finite-volume spectrum in a periodic $L \!\times\! L \!\times\! L$ box is encoded in the L\"uscher quantization condition,
\begin{equation}
\det \Big[ \bm{1} + i \bm{\rho} \, \bm{t} \, \big( \bm{1} + i \bm{\mathcal{M}} \big)  \Big] = 0, \label{luscher}
\end{equation}
and an extensive discussion of how the relationship can be implemented is presented in Ref.~\cite{Briceno:2017max}. Our approach is to make use of \emph{parameterizations} of the energy dependence of $\bm{t}(E_\mathsf{cm})$ and to attempt to describe as much of an obtained finite-volume lattice QCD spectrum as possible by varying the parameters in the parameterization, solving Eqn.~\ref{luscher} for the finite-volume spectrum for each choice of parameter values, and comparing to the lattice spectrum. An efficient method to solve the above equation, particularly applicable in cases of coupled-channels or coupled partial waves is presented in Ref.~\cite{Woss:2020cmp}.

An important feature of the above quantization condition is that it only has solutions for $t$-matrices which satisfy the unitarity condition that implements the conservation of probability. A straightforward way to ensure this is to make use of $K$-matrices by writing,
\begin{equation}
 \bm{t}^{-1} = \bm{K}^{-1} + \bm{I} \, , \label{tK}
\end{equation}
where $\bm{K}(s = E_\mathsf{cm}^2)$ is a symmetric real matrix in the space of coupled-channels and/or coupled partial waves, and where $\bm{I}(s)$ is a diagonal matrix with imaginary parts of value $\mathrm{Im}\, I_i(s) = - \rho_i(s)$, where the \emph{phase-space}, $\rho = \tfrac{2 k}{\sqrt{s}}$.
%
The real part of $I_i(s)$ can simply be chosen to be zero, in which case we speak of using the ``naive phase-space'', or we can make the choice to use the result of placing $\rho(s)$ in a dispersive integral, leading to what is often called the ``Chew-Mandelstam phase-space''. The dispersive integral is once-subtracted, and the location of the subtraction can be chosen for our convenience -- our implementation is described in Appendix B of Ref.~\cite{Wilson:2014cna}. 

We have significant freedom to choose parameterization forms for $\mathbf{K}(s)$, and a good approach is to try a range of parameterizations, finding as many as possible that can describe the finite-volume spectrum. If the resulting amplitude has features that are robust under changes of parameterization, we can be confident that they are true features of the actual QCD amplitude. This approach has been used extensively in previous calculations of elastic and coupled-channel scattering by the \emph{hadspec} collaboration~\cite{Dudek:2014qha,Wilson:2014cna,Wilson:2015dqa,Dudek:2016cru,Woss:2018irj,Woss:2019hse}.

%A very simple choice, using just a single pole in $\mathbf{K}$ leads to a Breit-Wigner like form. 

In practice, for scattering in partial waves with non-zero orbital angular momentum, $\ell$, we extract from the $K$-matrix the momentum factors needed to get the correct threshold behavior, writing
\begin{equation}
 \left[\bm{t}^{-1}\right]_{\ell \ell'} = \tfrac{1}{(2 k)^\ell} \left[\bm{K}^{-1}\right]_{\ell \ell'} \tfrac{1}{(2 k)^{\ell'}}  + \bm{I}, \label{tKk}
\end{equation}
for the case of two coupled partial waves ($\ell$, $\ell'$). Details of how dynamically coupled partial waves are handled in the $\ell S$ basis can be found in Refs.~\cite{Woss:2018irj, Woss:2019hse, Woss:2020ayi}.


Resonances in a scattering system are associated with \emph{pole singularities} at complex values of $s$ located on \emph{unphysical} Riemann sheets (those where the scattering momentum has a negative imaginary part). The real and imaginary parts of the pole position are commonly given meanings in terms of the mass and total width of the resonance, $\sqrt{s_0} = m \pm \tfrac{i}{2} \Gamma$, where the two signs reflect the fact that these poles always come in complex-conjugate pairs. Couplings to decay channels in each partial wave, $c_i$, can be obtained by factorizing the residue at the pole position,
\begin{equation*}
t_{ij}(s) \sim \frac{c_i \, c_j}{s_0 -s}.
\end{equation*}  

Poles can also lie on the real energy axis below the lowest kinematic threshold -- if they appear on the physical sheet they are associated with stable \emph{bound states} that can appear as asymptotic particles, while if they appear on unphysical sheets they are termed \emph{virtual bound states} which do not have an associated asymptotic particle.

The $t$-matrix can have other singularities, notably \emph{cuts} associated with the dynamics of scattering in crossed-channels. These are known as \emph{left-hand cuts}, and typically their effect on physical scattering is much milder than the effects of narrow resonances, and their net effect on physical scattering can be modelled by including slowly varying polynomial behavior in the $K$-matrix\,\footnote{But see Refs.~\cite{Briceno:2016mjc, Wilson:2019wfr} for cases where resonances may appear that are very broad and where the physics of the left-hand cut may become relevant.}. They are discussed further in the current context in Appendix~\ref{lhc}.

% ... introduction of left-hand cut concept here, or delay that until later ? poles on the physical sheet being acausal, bound state poles having to have a certain sign of residue
%\vspace{15cm}


We now proceed to present descriptions of the finite-volume spectra introduced in the previous section, beginning with the assumed elastic $\etaOctet \omegaOctet$ spectra of Figure~\ref{e8o8_spectra}, using parameterizations of elastic scattering in $J^{PC} = 1^{--}$, $2^{--}$ and $3^{--}$. We will consider several strategies to isolate the amplitudes, firstly considering those irreps which only depend upon scattering with $J^{PC}= 2^{--}$ and/or $3^{--}$, then those irreps which depend only upon $1^{--}$ and $3^{--}$, before finally attempting a global description of all the energy levels. %We will find compatible results for the amplitudes in all cases.

%%%%%%%%
\subsection{$\bm{J^{PC} = 3^{--}}$ from the $\bm{[000]\, A_2^-}$ irrep}
%%%%%%%%

The only partial wave expected to contribute in the $[000]\, A_2^-$ irrep at the energies we are considering is $\etaOctet \omegaOctet  \{ \threeFthree \}$, and the volume dependence of energy levels in the top right panel of Figure~\ref{e8o8_spectra} appears to be a canonical ``avoided level crossing'' indicating a narrow resonance near $a_t E_\mathsf{cm} \sim 0.43$. 

An elastic $K$-matrix featuring a single pole, ${K(s) = \frac{g^2}{m^2 -s} }$, and either a Chew-Mandelstam or naive phase-space is capable of describing this spectrum with a $\chi^2/N_\mathrm{dof} = \tfrac{5.2}{6-2}= 1.31$. The resulting amplitude has a narrow peak and no other features, and the $t$-matrix has a pole at ${a_t \sqrt{s_0} = 0.4296(16) \pm \tfrac{i}{2} 0.0027(8)}$ with a pole coupling of magnitude $a_t |c_{\etaOctet \omegaOctet}| = 0.047(7)$. Allowing additional freedom in the amplitude by adding a constant to the \mbox{$K$-matrix} leads to a negligible change in the quality of fit, and a consistent resonance pole.

From this analysis of a single irrep, it is clear that there is a narrow $3^{--}$ resonance -- we will delay providing further discussion until we report more a more precise determination of its pole parameters using a description of more energy levels.

%%%%%%%%
\subsection{$\bm{J^{PC} = 2^{--}}$ from the $\bm{[000]\, E^-}$ irrep}
%%%%%%%%

Assuming negligible $J=4$ scattering, the $[000]\, E^-$ irrep spectrum is controlled by the coupled partial waves, $\etaOctet \omegaOctet  \{ \threePtwo, \threeFtwo \}$, requiring a two-dimensional $t$-matrix,
\begin{equation*}
\bm{t} = \begin{bmatrix} t_{PP} & t_{PF} \\ t_{PF} & t_{FF}  \end{bmatrix}.
\end{equation*}

 Examining the volume dependence of energy levels in the second panel of Figure~\ref{e8o8_spectra}, we potentially observe an avoided level crossing with the lowest non-interacting $\etaOctet \omegaOctet$ curve, but spread out over a large energy range, which might signal a broad resonance somewhere around $a_t E_\mathsf{cm} \sim 0.42$. A simple amplitude that proves capable of describing this spectrum is given by the $K$-matrix,
\begin{equation}
%
\bm{ K}(s) = 
%
\frac{1}{m^2 - s} \begin{bmatrix} g_P^2 && g_P g_F \\ g_P g_F && g_F^2 \end{bmatrix} 
%
+ \begin{bmatrix} \gamma_{PP} && \gamma_{PF} \\ \gamma_{PF} && \gamma_{FF} \end{bmatrix},
%
\label{J2_pole_const}
\end{equation}
where when the Chew-Mandelstam phase-space is used (subtracted at $s=m^2$) in Eqn.~\ref{tKk}, the 13 energy levels can be described with a ${\chi^2/N_\mathrm{dof} = \tfrac{5.6}{13-6} = 0.80}$. The $t$-matrix in this case has a pole singularity at 
%
${a_t \sqrt{s_0} = 0.4181(30) \pm \tfrac{i}{2} 0.0325(77)}$,
%
and pole couplings to the two partial waves with magnitudes ${a_t |c_{\etaOctet \omegaOctet \{\threePtwo\} }| = 0.145(20)}$ and 
${a_t |c_{\etaOctet \omegaOctet \{\threeFtwo\} }| = 0.030(13)}$. As anticipated this single resonance has a significantly larger width than the one seen in $3^{--}$ and, as we'd expect for a resonance lying only slightly above the relevant decay threshold, the angular momentum barrier ensures an $F$--wave decay coupling that is significantly smaller than the leading $P$--wave.

A more precise determination of this $2^{--}$ amplitude, and of the $3^{--}$ amplitude discussed previously, can be obtained by simultaneously describing both in a description of the 91 finite-volume energy levels in the irreps $[000]\, A_2^-, T_2^-, E^-$ and $ [100]\, B_1, B_2$.

\newpage
%%%%%%%%
\subsection{$\bm{J^{PC} = 2^{--}, 3^{--}}$ from the $\bm{[000]\, A_2^-, T_2^-, E^-, [100]\, B_1, B_2}$ irreps}
%%%%%%%%

Five irreps, $[000]\, A_2^-, T_2^-, E^-$, and $[100]\, B_1, B_2$, are each sensitive to one or both of the $2^{--}$ and $3^{--}$ scattering amplitudes, and together feature 91 energy levels that we can use to constrain the energy dependence. As an example, using a single $K$-matrix pole for the $3^{--}$ amplitude, $K(s) = \frac{g^2}{m^2 -s}$, and the $K$-matrix presented in Eqn.~\ref{J2_pole_const} for the $2^{--}$ amplitude, with Chew-Mandelstam phase-space (subtracted at $s=m^2$) in both cases, we obtain a best-fit description of the finite-volume spectra with parameters,
\begin{widetext}
\vspace{0.5cm}
	\begin{center}
		\begin{tabular}{crll}
\ldelim\{{8.5}{*}[$J=2\,$]	&		$m =$  & $ 0.4322(15) \cdot a_t^{-1}$   &
			%%%%
			\multirow{9}{*}{ $\begin{bmatrix*}[r] 1 & 0.31 & 0.29  & 0.13  & -0.37 & 0.31  & 0.19  & 0.07 \\[1.1ex]
				                                    & 1    & -0.08 & -0.70 & 0.04  & 0.48  & 0.07  & -0.23 \\[1.1ex]
													&      & 1     & 0.21  & -0.15 & -0.18 & -0.01 & -0.12 \\[1.1ex]
													&      &       & 1     & -0.34 & -0.34 & -0.16 & 0.23 \\[1.1ex]
													&      &       &       & 1     & -0.23 & -0.03 & -0.05 \\[1.1ex]
													&	   &       &       &       & 1     & 0.02  & 0.05 \\[1.5ex]
													&      &       &       &       &       & 1     & -0.04 \\[1.1ex]
													&      &       &       &       &       &       & 1 \\[1.1ex]
													 \end{bmatrix*}$ } \\[1.1ex]
			%%%%	
&			$g_P  =$ & $ 0.753(37)  $   & \\[1.1ex]
&			$g_F =$ & $ -4.13(29) \cdot a_t^{2}$   & \\[1.1ex]
&			$\gamma_{PP} = $ & $0.1(33)\cdot a_t^{2}$   & \\[1.1ex]
&			$\gamma_{PF} = $ & $-110(17)\cdot a_t^{4}$   & \\[1.1ex]
&			$\gamma_{FF} = $ & $143(322)\cdot a_t^{6}$   & \\[1.5ex]
%
\ldelim\{{2.6}{*}[$J=3\, $]	&		$m =$  & $ 0.4341(9) \cdot a_t^{-1}$ \\[1.1ex]
  &			$g  =$ & $ 4.85(28) \cdot a_t^{2} $   & \\[2.5ex]
			%
			\multicolumn{4}{r}{$\chi^2/N_{\text{dof}}=\frac{120.3}{91 - 8}=1.45$\,.}
		\end{tabular}
	\end{center}
	\vspace{-1.1cm}
	%
	\begin{equation} \label{J2J3example}  \end{equation}
\end{widetext}

The fit quality is quite reasonable, and the parameters show no particularly large correlations. We observe that the constants $\gamma_{PP}, \gamma_{FF}$ are probably redundant, and later we will explore fixing them to zero. The resulting amplitudes are shown in Figure~\ref{2m3m_ref_rhotsq} where the bumps suggest the presence of a narrow resonance in $3^{--}$, and a broader resonance in $2^{--}$. The dominance of $\threePtwo$ over $\threeFtwo$ is obvious, and while the resonance bump is still visible in the off-diagonal element $t_{PF}$, albeit peaking at a slightly lower energy than in the $t_{PP}$ element, there is no clear peak in the weak $t_{FF}$ element.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 2m/3m reference fit  %%
\begin{figure}[b]
%
\includegraphics[width=0.98\columnwidth]{figures/2m3m_rhotsq_with_mayflies}
%
\caption{Scattering amplitudes for $J^{PC} = 2^{--}$ (Eqn.~\ref{J2_pole_const}) and $3^{--}$ ($K$-matrix pole), for the best-fit parameters of Eqn.~\ref{J2J3example}. Points below the abscissa show the positions of the finite-volume energy-levels constraining the amplitudes.
}
\label{2m3m_ref_rhotsq}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

These best-fit amplitudes feature $2^{--}$ and $3^{--}$ $t$-matrix poles that are compatible with those reported in previous sections in fits to $[000]\, E^-$, $[000]\, A_2^-$ alone, but which now have improved statistical uncertainty:
\begin{align*}
2^{--}: \quad\quad a_t \sqrt{s_0} &= 0.4235(18) \pm \tfrac{i}{2} 0.0375(34) \nonumber \\[1.2ex]
a_t c_{\etaOctet \omegaOctet\{ \threePtwo \}} &= 0.164(12) \, e^{\pm i \pi \, 0.13(2)} \nonumber \\
a_t c_{\etaOctet \omegaOctet\{ \threeFtwo \}} &= 0.057(6) \, e^{\mp i \pi \, 0.88(2)} \nonumber \\[2.2ex]
%
3^{--}: \quad\quad a_t \sqrt{s_0} &= 0.4338(9) \pm \tfrac{i}{2} 0.0049(6) \nonumber \\[1.2ex]
a_t c_{\etaOctet \omegaOctet\{ \threeFthree \}} &= 0.062(4) \, e^{\pm i \pi \, 0.038(5)} \, .
\end{align*}
We note that the $F$--wave couplings for the $2^{--}$ and $3^{--}$ resonances are of a very similar size. The $2^{--}$ resonance pole (in the lower half plane) has a ratio of $F$--wave to $P$--wave couplings of $0.35(3)\, e^{ i \pi \, 1.01(2)} \approx -0.35(3)$, which is close to being real and negative.

In order to establish that these results are not overly sensitive to details of the particular amplitude parameterization selected, we also explore descriptions of the finite-volume spectra using other choices, which include: replacing the Chew-Mandelstam phase-space with the naive phase space, setting some of the constants added to the $K$-matrix pole in Eqn.~\ref{J2_pole_const} to zero, replacing some of the constants with terms of form $\gamma\! \cdot\! s$, using a second pole in place of the constants, or by writing $\bm{K}^{-1}$ as a matrix of polynomials. The forms used are listed in Table~\ref{2mm_amps} in Appendix~\ref{par}. The resulting $2^{--}$ amplitudes\,\footnote{The $3^{--}$ amplitudes show completely negligible variation.} are shown in Figure~\ref{2m_variation_rhotsq}, and it is quite clear that the amplitude previously presented in Figure~\ref{2m3m_ref_rhotsq} is representative, and in fact it has among the largest statistical uncertainties of those amplitudes considered. While the bulk of the amplitudes tried have a $\chi^2/N_\mathrm{dof}$ very close to the value $1.45$ obtained using Eqn.~\ref{J2_pole_const}, there are three choices that have somewhat larger values: Eqn.~\ref{J2_pole_const} with $\gamma_{PF}$ fixed to zero ($\chi^2/N_\mathrm{dof} = 1.85$), a $K$-matrix built as the sum of two poles ($\chi^2/N_\mathrm{dof} = 1.80$), and a form where $\bm{K}^{-1}$ is parameterized as independent linear polynomials ($a+ b s$) in each element ($\chi^2/N_\mathrm{dof} = 1.67$). These outliers are shown by the dashed lines in Figure~\ref{2m_variation_rhotsq}, where we note that they have a slight difference in $t_{PP}$ peak position, but otherwise only start to show significant deviation from the solid curves above the energy region where constraint is provided by the finite-volume spectra.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 2m variations  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/2m_rhotsq_variation}
%
\caption{Variation of $2^{--}$ amplitude over parameterization choice. Solid curves and bands show descriptions of the finite-volume spectra with $1.42 < \chi^2/N_\mathrm{dof} < 1.46$, while dashed curves have $1.66 < \chi^2/N_\mathrm{dof} < 1.86$.}
\label{2m_variation_rhotsq}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 2m poles  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/2m_poles_variation}
\includegraphics[width=0.98\columnwidth]{figures/2m_couplings_variation}
\includegraphics[width=0.98\columnwidth]{figures/2m_R_variation}
%
\caption{Top panel: $2^{--}$ $t$-matrix pole positions for parameterization variations shown in Figure~\ref{2m_variation_rhotsq} -- black points show the fits with $1.42 < \chi^2/N_\mathrm{dof} < 1.46$ and grey those with $1.66 < \chi^2/N_\mathrm{dof} < 1.86$. Middle panel: the couplings, $c_{\etaOctet \omegaOctet \{\threePtwo\}}$ (green) and $c_{\etaOctet \omegaOctet \{\threeFtwo\}}$ (sand) obtained from factorizing the residue of the $t$-matrix pole in the lower half-plane -- lighter points show those fits with  poorer $\chi^2$. Bottom panel: The magnitude of the ratio of the couplings.}
\label{2m_variation_pole}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{2m_variation_pole} shows the $t$-matrix pole positions and the corresponding pole couplings for the parameterization variations, indicating a clear consensus that agrees with the reference amplitude described previously.
%
The amplitudes considered do have other pole singularities in addition to the one presented in Figure~\ref{2m_variation_pole}, but they are typically distant from physical scattering and vary with parameterization choice. A typical example, present in the reference amplitude, is a pole on the real axis on the unphysical sheet near $a_t \sqrt{s} \sim 0.23$ -- such a pole is present for many of our amplitudes, although its precise position varies, always remaining far from physical scattering, and as such it remains largely irrelevant to physical scattering. As one might expect given its inferior analytic properties, using the naive phase-space in place of the Chew-Mandelstam function leads to additional singularities, in particular a physical sheet pole on the real energy axis at $a_t \sqrt{s} \sim 0.24$ which is found to have \emph{real-valued} couplings. In odd-$\ell$ scattering, a true bound-state must have imaginary couplings, so the presence of this pole signifies a \emph{ghost} state having negative probability. Such a singularity suggests a flaw in the parameterization, but in practice the ghost pole is so far from physical scattering that it has a negligible impact -- we will further discuss such poles, and their relation to neglected left-hand cuts later, in the context of $1^{--}$ scattering\,\footnote{A ghost pole in $S$-wave is the pathology that causes an amplitude to fail the `sanity check' of Iritani \emph{et.al.}~\cite{Iritani:2017rlk}.}.
%. 

The case of an amplitude in which $\bm{K}^{-1}$ is parameterized with linear functions features a different pathology: there are poles \emph{off the real axis on the physical sheet}, albeit fairly deep into the complex plane. Such poles signal a breakdown in \emph{causality} which comes about because we do not place analyticity constraints upon our amplitudes.





We will later return to further discussion of the $2^{--}$ and $3^{--}$ amplitudes in the context of a global analysis of all of our finite-volume energies levels, while now we move to an initial determination of the $J^{PC} = 1^{--}$ amplitude.


%%%%%%%%
\subsection{$\bm{J^{PC} = 1^{--}, 3^{--}}$ from the $\bm{ [000]\, T_1^-,\, [100]\, A_1,\, [111]\, A_1 }$ irreps}
%%%%%%%%

Irreps $[000]\, T_1^-, [100]\, A_1$, and $[111]\, A_1$ all depend upon both the $1^{--}$ and the $3^{--}$ amplitude, but not the $2^{--}$ amplitude. Since we have a well-constrained $3^{--}$ amplitude from the previous subsection, we choose to initially fix this amplitude, and only vary the $1^{--}$ amplitude. We will relax this later when we attempt descriptions of our entire set of finite-volume energy levels.

We will not try to include the very deeply-bound stable $\omegaSinglet$ as an explicit pole in our scattering amplitudes, and hence we exclude the lowest energy level in each irrep on each volume. There are 72 suitable energy levels below $a_t E_\mathsf{cm} = 0.46$ shown in Figure~\ref{e8o8_spectra}, and as discussed in Section~\ref{fvspectrum} and shown in Figure~\ref{T1m_histo}, the spectra and operator overlaps hint at there being two $1^{--}$ resonances present. Narrow resonances are most conveniently parameterized by including explicit poles in the $K$-matrix, and as such a good choice of amplitude to illustrate this case features two poles and a constant, where the constant allows for some flexibility away from a pure superposition of resonances. The Chew-Mandelstam phase-space, subtracted at the lower mass pole ($s=m_\mathsf{a}^2$) is used, and the best fit parameters are found to be,
\vspace{0.1cm}
	\begin{center}
		\begin{tabular}{rll}
 $m_\mathsf{a} =$  & $ 0.3881(14) \cdot a_t^{-1}$   &
			%%%%
			\multirow{5}{*}{ $\begin{bmatrix*}[r] 1 & 0.08  & 0.43  & -0.33  & 0.19  \\[1.1ex]
				                                    & 1     & 0.37  & -0.46  & 0.81  \\[1.1ex]
													&       & 1     & -0.86  & 0.49  \\[1.1ex]
													&       &       & 1      & -0.57 \\[1.1ex]
													&       &       &        & 1     \\[1.1ex]
													 \end{bmatrix*}$ } \\[1.1ex]
			%%%%	
			$g_\mathsf{a} = $ &  $ 1.46(10)    $   & \\[1.1ex]
			$m_\mathsf{b} = $ &  $ 0.4242(17) \cdot a_t^{-1} $   & \\[1.1ex]
			$g_\mathsf{b} = $ &  $-0.36(13) $    & \\[1.1ex]
			$\gamma       = $ &  $20.9(86)    \cdot a_t^2$    & \\[2.2ex]
%
&			\multicolumn{2}{r}{$\chi^2/N_{\text{dof}}=\frac{91.3}{72 - 5}=1.36$\,.}
		\end{tabular}
	\end{center}
	\vspace{-0.5cm}
	%
	\begin{equation} \label{J1example}  \end{equation}
The description is reasonable, and we note that the parameter correlations are modest, with the constant $\gamma$ being statistically significant. The resulting amplitude is shown in Figure~\ref{1m_ref_rhotsq} where we observe a prominent dip with a zero located at $a_t E_\mathsf{cm} = 0.4216(9)$. The points shown beneath the abscissa show the positions of the energy levels used to constrain the amplitude, which cover the entire energy region of interest. When the $t$-matrix is examined in the complex $s$-plane, two pole singularities are found close to the real axis on the unphysical sheet:
\begin{align*}
a_t \sqrt{s_0} &= 0.3787(16) \pm \tfrac{i}{2} 0.0187(13) \nonumber \\[1.1ex]
a_t c_{\etaOctet \omegaOctet\{ \threePone \}} &= 0.144(4) \, e^{\pm i \pi \, 0.202(17)} \, ,
\end{align*}
%
and 
%
\begin{align*}
a_t \sqrt{s_0} &= 0.4224(8) \pm \tfrac{i}{2} 0.0030(20) \nonumber \\[1.1ex]
a_t c_{\etaOctet \omegaOctet\{ \threePone \}} &= 0.051(17) \, e^{\pm i \pi \, 0.352(27)} \, .
\end{align*}

\newpage
We interpret these two $t$-matrix poles as being the signal for two $1^{--}$ resonances, a lighter broader state, and a heavier narrow state. The zero on the real energy axis is located close to the second resonance pole\,\footnote{
There is guaranteed to be a zero located between $s= m_\mathsf{a}^2$ and $s= m_\mathsf{b}^2$ whenever a two-pole plus polynomial form is used for an \emph{elastic} $K$-matrix. 

Since $t = \tfrac{K}{1+ I K}$ and $K(s) = \tfrac{g_\mathsf{a}^2}{m_\mathsf{a}^2 - s} + \tfrac{g_\mathsf{b}^2}{m_\mathsf{b}^2 - s} + \gamma(s)$, defining $P(s) = (m_\mathsf{a}^2 - s)(m_\mathsf{b}^2 - s) K(s)$ we have $t(s) = \tfrac{P(s)}{ (m_\mathsf{a}^2 - s)(m_\mathsf{b}^2 - s) + I(s) P(s)} $ and a zero of $t(s)$ will appear when $P(s)=0$. Since $P(m_\mathsf{a}^2) = g_\mathsf{a}^2 ( m_\mathsf{b}^2 - m_\mathsf{a}^2) > 0$ and ${ P(m_\mathsf{b}^2) = - g_\mathsf{b}^2 ( m_\mathsf{b}^2 - m_\mathsf{a}^2) < 0 }$, $P(s)$ must cross zero at least once between $s=m_\mathsf{a}^2$ and $s=m_\mathsf{b}^2$. If $g_\mathsf{b}$ is small, it is clear that $P(m_\mathsf{b}^2)$ will have a value close to zero and hence the zero of $t(s)$ will be close to $s= m_\mathsf{b}^2$.
}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1m reference fit  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/1m_rhotsq}
%
\caption{Illustrative two-pole plus constant $\etaOctet \omegaOctet \{\threePone \}$($1^{--}$) elastic scattering amplitude (Eqn.~\ref{J1example}). Points below the abscissa show the positions of the finite-volume energy-levels constraining the amplitudes.
}
\label{1m_ref_rhotsq}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Elastic unitarity is a strong constraint that significantly restricts the possible behavior of an amplitude like this, and as seen in Figure~\ref{1m_ref_rhotsq}, there is clearly a non-trivial energy dependence, one that does not for example simply consist of two separated bumps as one might anticipate given the resonance content. This is one reason why the use of complex $s$-plane pole positions is advocated as a rigorous identification of resonances -- one could not describe this amplitude as a sum of two Breit-Wigners.

%We note the relatively slow fall-off of the amplitude above the second resonance. The presence of an explicit factor of $(2k)^{2\ell}$ in the relationship between $t$ and $K$, Eqn.~\ref{tKk}, will tend to cause growth of $t(s)$ at high energies, and a common approach in fitting of experimental data is to tame this with \emph{barrier factors}. A particularly simple barrier model for elastic scattering in a single partial wave has
%\begin{equation}
%t^{-1}_\ell(s) = \frac{(s+s_L)^{2 \ell +\alpha}}{(2k)^{2\ell}} K_\ell^{-1}(s) + I(s), \label{simple_barrier}
%\end{equation}
%where $s_L$ provides an energy scale for the barrier fall-off, and where increasing values of $\alpha$ will strengthen the damping effect. As the $t$-matrix will now contain a pole at $s = - s_L$, a slightly improved model is to consider that pole to be part of the left-hand cut, and to implement it into an approximation of an ``$N/D$'' dispersion relation,
%\begin{align}
%t_\ell(s) &= \frac{N_\ell(s)}{D_\ell(s)} \nonumber \\
%D_\ell(s) &= \frac{1}{(2k)^{2\ell}} K_\ell^{-1}(s) - \frac{s-s_0}{\pi} \int_{s_\mathrm{thr.}}^\infty \!\!\!\! ds' \, \frac{ \rho(s') N_\ell(s') }{(s'-s-i\epsilon)(s'-s_0)} \nonumber \\
%N_\ell(s) &= \frac{1}{(s+s_L)^{2\ell +\alpha} }, \label{ND}
%\end{align}
%with the expectation that the analytical properties of the resulting amplitude should be somewhat improved~\footnote{more discussion can be found in Appendix XXX}.



We now move to explore whether the same finite-volume spectrum can be described by other choices of amplitude parameterization, and whether the resulting amplitudes have the same features as just observed. Variations considered include varying the choice for $I(s)$, by changing the subtraction point or by simply using the naive phase-space, and varying what kind of polynomial is added to the two $K$-matrix poles. Table~\ref{1mm_amps} in Appendix~\ref{par} lists the variations, and in Figure~\ref{1m_rhotsq_variation} we show the amplitudes obtained using these parameterization variations, all of which prove capable of describing the finite-volume spectra with ${\chi^2 / N_\mathrm{dof} < 1.44}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1m variations  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/1m_rhotsq_variation_polish}
%
\caption{
Variation of $1^{--}$ amplitude over parameterization choice. Dashed curves show cases with just two poles in the $K$-matrix and no further freedom.
}
\label{1m_rhotsq_variation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
We note that there is very little observed change in the amplitude except at the highest energies, and in particular the location of the zero in the amplitude appears to be very stable. We display two examples of allowing too little freedom in the amplitude -- the dashed curves show parameterizations featuring only two $K$-matrix poles and no further freedom with either the Chew-Mandelstam phase-space subtracted at the lower pole, or the naive phase-space. We see that they are compatible with the other parameterizations in the region of the resonances, but deviate at high energy. Our conclusion is that some freedom beyond two poles in the $K$-matrix is needed to have the amplitude fall-off at higher energy -- adding a constant seems to be sufficient. 



%We note that in those cases where we implement barrier factors, either in the simple form, or dispersively improved, the $K$-matrix parameters tend to adjust themselves to compensate for the imposed barriers, suggesting that the plotted rate of fall-off reflects that required by the finite-volume spectra and is not an unwanted consequence of  our particular $K$-matrix parameterization choices.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1m variations  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/1m_delta_variation_polish}
%
\caption{Elastic scattering phase-shift for $1^{--}$, variation over parameterization choice. Dashed curves show cases with just two poles in the $K$-matrix and no further freedom.
}
\label{1m_delta_variation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




Because this process is elastic, we can alternatively display the scattering in terms of an elastic phase shift, $\delta(E_\mathsf{cm})$ , defined by $t = \tfrac{1}{\rho} e^{i \delta} \sin \delta$. The classic signal for an isolated narrow resonance is a rapid rise of $\delta$ passing through $90^\circ$, with the steepness of the rise correlated with the smallness of the resonance width. As observed in Figure~\ref{1m_delta_variation}, the phase shift undergoes two such increases, the first with a low slope and the second being much more rapid. The phase shift passing through $180^\circ$ represents the zero in the amplitude, and the relatively slow approach to $360^\circ$ reflects the slow fall off of the amplitude at high energy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1m poles  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/1m_poles_variation_polish}
%
\includegraphics[width=0.98\columnwidth]{figures/1m_couplings_variation_polish}
%
\caption{
Top panel: $1^{--}$ $t$-matrix pole positions for parameterization variations shown in Figures~\ref{1m_rhotsq_variation},\ref{1m_delta_variation}.  Bottom panel: the coupling, $c_{\etaOctet \omegaOctet \{\threePone\}}$ obtained from factorizing the residue of the $t$-matrix poles in the lower half-plane. Gray points represent the amplitudes having limited freedom shown by the dashed curves in Figures~\ref{1m_rhotsq_variation},\ref{1m_delta_variation}.
}
\label{1m_poles_variation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{1m_poles_variation} shows the location of the two $t$-matrix pole singularities and their pole couplings for all the parameterization variations considered. It is clear that there is very little scatter, and that robust conclusions can be drawn about these two resonances appearing in $1^{--}$. Additional pole singularities which lie further from physical scattering are found for some of amplitude variations, in particular several parameterizations feature an extra unphysical sheet pole, lying slightly above the energy region that we have constrained and far into the complex plane. As shown in Figure~\ref{1m_all_poles_variation}, its position is not well determined, and indeed it is not present in all parameterizations, and as such it appears to be an irrelevant artifact\,\footnote{The anticipated $1^{--}$ hybrid meson resonance pole is expected to lie at a somewhat larger energy, and is unlikely to be well constrained without higher-lying energy levels being included in the analysis.}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1m poles  %%
\begin{figure}[b]
%
\includegraphics[width=0.98\columnwidth]{figures/1m_all_poles_variation_polish}
%
\caption{As in Figure~\ref{1m_poles_variation}, the $1^{--}$ $t$-matrix pole positions for parameterization variations shown in Figure~\ref{1m_rhotsq_variation}, including a poorly determined pole at higher energy (red).
}
\label{1m_all_poles_variation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another additional pole singularity is present for several parameterizations, lying on the real energy axis below threshold on the physical sheet. Whenever it appears it is found to have a \emph{real-valued} coupling, indicating that is is a \emph{ghost}. In our illustrative amplitude with two \mbox{$K$-matrix} poles and a constant using Chew-Mandelstam phase-space, it is located at $a_t \sqrt{s} = 0.278(26)$, and it is quite typical across parameterization variations that it lies well below threshold. Such a location is into the left-hand cut region (as discussed in Appendix~\ref{lhc}), and we might interpret the presence of this ghost pole as reflecting the fact that we have made no attempt to parameterize the correct structure of the left-hand cut.

%It is worth singling out here one particular parameterization. Using the simple barrier model presented above in Eqn.~\ref{simple_barrier} (with $\alpha = 1$) and just two $K$-matrix poles with the naive phase-space  might be a natural phenomenological description of a scattering system featuring two resonances. This amplitude can reproduce the two \mbox{$t$-matrix} poles we have associated with resonances, but it also has a ghost pole lying at $a_t \sqrt{s} = 0.3403(22)$, which is rather close to physical scattering, and which it is hard to justify ignoring as due to a neglected left-hand cut. The dispersively improved barriers move this ghost pole much further away, so this result may reflect poor analytic properties of the simple barrier model.

The analyses in the last few sections, considering a subset of all computed irreps each time, has led to a clear picture of the resonance content of the $1^{--}, 2^{--}, 3^{--}$ partial-waves up to an energy $a_t E_\mathsf{cm} \sim 0.46$. We have not so far made any use of the $[110]\, A_1$ irrep which depends upon the scattering amplitudes of \emph{all} the above partial waves. We will now move to consider a global fit of all the $\etaOctet \omegaOctet$ energy levels that will confirm the results seen so far, and lead to reduced statistical uncertainties on some resonance parameters.


%%%%%%%%
\subsection{`Global fit' to all $\bm{ \etaOctet \omegaOctet }$ energy levels} \label{global}
%%%%%%%%

%{\color{jlab_red} include anisotropy variation in here}

In this section we attempt a description of the full set of 192 energy levels shown in black in Figure~\ref{e8o8_spectra} using parameterizations of $1^{--}$, $2^{--}$ and $3^{--}$ scattering amplitudes. To illustrate the approach we select amplitudes where $3^{--}$ is described by a single $K$-matrix pole with Chew-Mandelstam phase-space subtracted at the pole, the $2^{--}$ $\threePtwo, \threeFtwo$ coupled system is described by a \mbox{$K$-matrix} pole plus constants in the $PP$ and $PF$ positions with Chew-Mandelstam phase-space subtracted at the pole, and $1^{--}$ is described by two $K$-matrix poles plus a constant with Chew-Mandelstam phase-space subtracted at the lower pole. A description of the complete set of energy levels is found with $\chi^2/N_\mathrm{dof} = 258.3/(192-12) = 1.43$, and the finite-volume spectrum following from the best-fit amplitude is shown by the orange curves in Figure~\ref{e8o8_orange}. As we might guess from the relatively small $\chi^2$, the orange curves are in good agreement with the black points. While the spectrum of `predicted' levels can be dense, it always agrees with our expectations of the number of levels arising from non-interacting levels plus resonances, once multiple subductions are accounted for -- as an example, consider small volumes in the $[110]\,A_1$ irrep, where the six orange curves agrees with an expectation based upon one low-lying $\etaOctet \omegaOctet$ non-interacting level and five resonance contributions ($1^{--}_\mathsf{a}$, $1^{--}_\mathsf{b}$, $2^{--}$, and $3^{--}$ subduced twice). We note that in cases where resonances in different $J^{PC}$ overlap, the ``avoided level crossing'' structure can be somewhat non-trivial.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1m global amplitude  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/1m2m3m_rhotsq_with_mayflies}
%
\caption{
$\etaOctet \omegaOctet$ elastic scattering amplitudes obtained by describing 192 finite-volume energy levels.
}
\label{1m2m3m}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% e8o8 spectra %%
\begin{figure*}
%
\includegraphics[width=0.95\textwidth]{figures/restframe_orange}
\includegraphics[width=0.95\textwidth]{figures/inflight_orange}
%
\caption{Spectra from Figure~\ref{e8o8_spectra} used to constrain $\etaOctet \omegaOctet$ elastic scattering amplitudes. Orange curves show the finite-volume spectrum corresponding to the best-fit amplitudes. For guidance, the purple ($1^{--}$), green ($2^{--}$) and cyan ($3^{--}$) bands show the resonance masses and widths, allowing avoided level crossings to be observed with the non-interacting $\etaOctet \omegaOctet$ levels (red dashed).}
\label{e8o8_orange}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



The amplitudes are shown in Figure~\ref{1m2m3m} where they are seen to be compatible with our previous determinations using subsets of the spectrum. The $t$-matrices are found to feature poles on the unphysical sheet at the following locations (and with pole couplings):
\begin{align}
1^{--}(\mathsf{a}): \quad\quad a_t \sqrt{s_0} &= 0.3806(12) \pm \tfrac{i}{2} 0.0181(12) \nonumber \\[1.2ex]
a_t c_{\etaOctet \omegaOctet\{ \threePone \}} &= 0.141(5) \, e^{\pm i \pi \, 0.18(1)} \nonumber \\[2.2ex]
%
1^{--}(\mathsf{b}): \quad\quad a_t \sqrt{s_0} &= 0.4230(7) \pm \tfrac{i}{2} 0.0032(16) \nonumber \\[1.2ex]
a_t c_{\etaOctet \omegaOctet\{ \threePone \}} &= 0.052(13) \, e^{\pm i \pi \, 0.34(2)} \nonumber \\[2.2ex]
%
2^{--}: \quad\quad a_t \sqrt{s_0} &= 0.4242(10) \pm \tfrac{i}{2} 0.0391(24) \nonumber \\[1.2ex]
a_t c_{\etaOctet \omegaOctet\{ \threePtwo \}} &= 0.175(5) \, e^{\pm i \pi \, 0.11(1)} \nonumber \\
a_t c_{\etaOctet \omegaOctet\{ \threeFtwo \}} &= 0.059(4) \, e^{\mp i \pi \, 0.88(2)} \nonumber \\[2.2ex]
%
3^{--}: \quad\quad a_t \sqrt{s_0} &= 0.4342(6) \pm \tfrac{i}{2} 0.0052(5) \nonumber \\[1.2ex]
a_t c_{\etaOctet \omegaOctet\{ \threeFthree \}} &= 0.064(3) \, e^{\pm i \pi \, 0.040(4)} \, . \label{global_poles}
\end{align}
These are compatible with those found previously. 

Thus far we have not accounted for the effect of the (relatively small) uncertainties on the scattering hadron \mbox{($\etaOctet$, $\omegaOctet$)} masses on the scattering amplitudes, but when considered by varying them by $\pm 1 \sigma$, there is negligible change. The somewhat larger conservative estimate of the uncertainty on the anisotropy, $\xi = 3.486(43)$, has only been accounted for partly, in the boost of moving frame energies back to $a_t E_\mathsf{cm}$. It can also be considered in the computation of $\bm{\mathcal{M}}$ in Eqn.~\ref{luscher}, where varying by $\pm 1 \sigma$ leads to small adjustments in the pole positions given above. The largest effects are observed in the real part of the pole positions which can move by amounts comparable with the statistical error, and in the imaginary part of the $2^{--}$ pole position. In the next section, when we present our best estimates for the resonance pole properties we will include this source of uncertainty in our error estimates.

%... can consider the effect of the uncertainties on the scattering hadron masses and the anisotropy ... anisotropy is the largest effect ... give or at least comment on the increase in uncertainty ... compare with the variational over parameterizations ... comment that our estimate is likely to be very conservative ...



%\newpage
%%%%%%%%
\subsection{Decoupled $\bm{\etaSinglet \omegaSinglet}$ and $\bm{ \omegaSinglet \fZeroSinglet }$ scattering}
%%%%%%%%

As discussed in Section~\ref{fvspectrum}, the finite-volume spectrum appears to separate into a spectrum due to the resonating $\etaOctet \omegaOctet$ system that we have just considered, and two spectra due to non-resonant systems $\etaSinglet \omegaSinglet$ and $\omegaSinglet \fZeroSinglet$. We will consider these latter sets of energy levels in isolation. 

For $J^{PC} = 1^{--}$ $\etaSinglet \omegaSinglet \{ \threePone \}$ elastic scattering, we use five energy levels as constraint, three levels in $[000]\, T_1^-$ (as shown in the bottom panel of Figure~\ref{T1m_histo}) and two in $[001]\, A_1$, all of which are compatible with lying on the lowest non-interacting $\etaSinglet \omegaSinglet$ curve.

An effective range expansion $k^3  \cot \delta = \tfrac{1}{a} + \tfrac{1}{2} r k^2 + \ldots$ can be used to describe the elastic amplitude. Using only a scattering length $a \neq 0, r = 0$ and no higher terms in the polynomial, the five energy levels can be described with $a = 4.4(40) \times 10^2\, a_t^3$ with a ${\chi^2/N_\mathrm{dof} = 6.2/(5-1) = 1.5 }$. Such a $P$--wave scattering length approximation gives a \mbox{$t$-matrix} pole distribution that is not easily interpreted (three poles evenly spaced around a circle of radius ${k = a^{-1/3}}$), but allowing also a non-zero effective range, which can generate a realistic pole distribution in this case leads to a fit with 100\% correlation between the parameters ($a,r$). 

Alternatively, using a constant $K$-matrix and the Chew-Mandelstam phase-space subtracted at threshold, the energy levels can be described with a ${\chi^2/N_\mathrm{dof} = 6.1/(5-1) = 1.5}$ where the resulting \mbox{$t$-matrix} has a \emph{ghost} pole on the physical sheet at ${  a_t \sqrt{s_0} = 0.315(78)  }$ -- given that the left-hand cut for this process begins at $0.378$ (see Appendix~\ref{lhc}), we can associate this ghost with our lack of control over the crossed-channel physics.

For $J^{PC} = 2^{--}$, assumed to be only in the $\etaSinglet \omegaSinglet \{ \threePtwo \}$ partial wave, we use 8 levels from $[000]\, E^-$, $[000]\, T_2^-$, and $[001]\, B_1$. The $F$--wave $3^{--}$ amplitude is assumed to be negligible. A scattering length description finds ${ a = 4.1(28) \times 10^2\, a_t^3 }$ with a ${ \chi^2/N_\mathrm{dof} = 12.7/(8-1) = 1.8 }$, while a constant $K$-matrix with Chew-Mandelstam subtracted at threshold has a similar $\chi^2$ and a ghost pole at $a_t \sqrt{s_0} = 0.305(73)$.

It is clear that the partial waves $\etaSinglet \omegaSinglet \{ \threePone, \threePtwo \}$ are non-resonant -- the elastic phase-shift reaches only $\sim 20^\circ$ at the largest energies we consider ($a_t E_\mathsf{cm} \sim 0.46$) -- and they appear to have very similar behavior suggesting weak spin-orbit forces in this channel. The large uncertainties on the scattering parameters are only slightly increased if we include the effect of the uncertainty on the $\etaSinglet$ mass.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For $J^{PC} = 1^{--}$ $\omegaSinglet \fZeroSinglet$, we in principle may have a more significant amplitude, owing to the scattering being possible in an $S$--wave ($\threeSone$). In fact a coupled system of partial waves $\{ \threeSone, \threeDone \}$ is required in order to describe the multiplicity of non-interacting energies shown in the middle panel of Figure~\ref{T1m_histo}. We make use of 16 energy levels taken from $[000]\, T_1^-$ and $[001]\, A_1$ irreps, noting that they all have rather large statistical uncertainties and are all compatible with non-interacting $\omegaSinglet \fZeroSinglet$ energies.

An example parameterization uses a diagonal constant $K$-matrix and a Chew-Mandelstam phase-space subtracted at threshold. The resulting constants are statistically compatible with zero in a description of the energy levels with $\chi^2/N_\mathrm{dof} = 21.5/(16-2) = 1.54$. Even larger errors are obtained once the uncertainty on the $\fZeroSinglet$ mass is accounted for, and considering this and variation over parameterizations, the $S$--wave phase-shift remains compatible with zero but with an uncertainty that spreads over at least $\pm 50^\circ$ at $a_t E_\mathsf{cm} = 0.46$. 


%%%%%%%%
\subsection{Estimating coupled-channel effects}
%%%%%%%%

The previous sections indicate that the finite-volume spectra can be well described assuming that the $\etaOctet \omegaOctet$, $\etaSinglet \omegaSinglet$, and $\omegaSinglet \fZeroSinglet$ channels are decoupled, with resonances only appearing in $\etaOctet \omegaOctet$. Nevertheless we can attempt a limited study of possible channel coupling.

Using a set of 52 energy levels in irreps sensitive to $J^{PC}=1^{--}$ and $3^{--}$, which includes 4 levels having large $\etaSinglet \omegaSinglet$ overlap, we can try to constrain coupled $(\etaOctet \omegaOctet, \etaSinglet \omegaSinglet)$ $J^{PC} = 1^{--}$ amplitudes parameterized with
\begin{align}
\bm{K}(s) &= 
%
\frac{1}{m_\mathsf{a}^2 - s} 
\begin{bmatrix} 
(g^{\mathsf{a}}_{\etaOctet \omegaOctet})^2 & g^{\mathsf{a}}_{\etaOctet \omegaOctet}\, g^{\mathsf{a}}_{\etaSinglet \omegaSinglet}\\ 
g^{\mathsf{a}}_{\etaOctet \omegaOctet}\, g^{\mathsf{a}}_{\etaSinglet \omegaSinglet} & (g^{\mathsf{a}}_{\etaSinglet \omegaSinglet})^2 
\end{bmatrix} 
\nonumber \\
%
&\;\;+ \frac{1}{m_\mathsf{b}^2 - s} 
\begin{bmatrix} 
(g^{\mathsf{b}}_{\etaOctet \omegaOctet})^2 & g^{\mathsf{b}}_{\etaOctet \omegaOctet}\, g^{\mathsf{b}}_{\etaSinglet \omegaSinglet}\\ 
g^{\mathsf{b}}_{\etaOctet \omegaOctet}\, g^{\mathsf{b}}_{\etaSinglet \omegaSinglet} & (g^{\mathsf{b}}_{\etaSinglet \omegaSinglet})^2 
\end{bmatrix} 
\nonumber \\
%
&\qquad\qquad\;  + \begin{bmatrix} \gamma_{\etaOctet \omegaOctet, \etaOctet \omegaOctet } & \gamma_{\etaOctet \omegaOctet, \etaSinglet \omegaSinglet } \\ \gamma_{\etaOctet \omegaOctet, \etaSinglet \omegaSinglet } & \gamma_{\etaSinglet \omegaSinglet, \etaSinglet \omegaSinglet } \end{bmatrix},
%
\label{coupled}
\end{align}
and Chew-Mandelstam phase-space subtracted at $s=m_\mathsf{a}^2$. The $J^{PC} = 3^{--}$ amplitude is a single $K$-matrix pole, elastic in $\etaOctet \omegaOctet$ with parameters fixed from previous fits.

In practice the $\mathsf{a}$--pole being far below $\etaSinglet \omegaSinglet$ threshold means that the parameter $g^{\mathsf{a}}_{\etaSinglet \omegaSinglet}$ is basically unconstrained so we set it equal to zero. $\gamma_{\etaSinglet \omegaSinglet, \etaSinglet \omegaSinglet }$ is always left free, and we consider three fits:
\begin{align}
g^{\mathsf{b}}_{\etaSinglet \omegaSinglet} \neq 0&, \gamma_{\etaOctet \omegaOctet, \etaSinglet \omegaSinglet } = 0 , \nonumber\\
g^{\mathsf{b}}_{\etaSinglet \omegaSinglet}  = 0&, \gamma_{\etaOctet \omegaOctet, \etaSinglet \omegaSinglet } \neq 0, \nonumber \\
g^{\mathsf{b}}_{\etaSinglet \omegaSinglet} \neq 0&, \gamma_{\etaOctet \omegaOctet, \etaSinglet \omegaSinglet } \neq 0,  
\label{coupled2}
\end{align}
all three of which provide descriptions of the energy levels with $\chi^2 /N_\mathrm{dof} = 1.84$. The resulting amplitudes are shown in Figure~\ref{1m_coupled} where we see that only the $t_{\etaOctet\omegaOctet, \etaOctet \omegaOctet}$ element is significantly non-zero in each case, and that it broadly agrees with the previous elastic analysis. The third fit is somewhat optimistic given the small number of $\etaSinglet \omegaSinglet$ dominated energy levels providing constraint, and indeed it is this amplitude that shows the largest difference with respect to the elastic case, in particular with it having the largest shift in the dip position. 

%... but notice that the position of the dip (and whether it goes all the way down to zero) can change relative to the elastic-only assumption ...


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1m coupled  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/1m_coupled}
%
\caption{Coupled $(\etaOctet \omegaOctet, \etaSinglet \omegaSinglet)$ $1^{--}$ amplitudes as in Eqns.~\ref{coupled}, \ref{coupled2}. $t_{\etaOctet \omegaOctet, \etaOctet \omegaOctet}$ (purple), $t_{\etaOctet \omegaOctet, \etaSinglet \omegaSinglet}$ (blue), $t_{\etaSinglet \omegaSinglet, \etaSinglet \omegaSinglet}$ (cyan). For comparison the assumed elastic amplitude from Figure~\ref{1m_ref_rhotsq} is shown in grey. The energy levels used to constrain the amplitude are shown below the abscissa, with those having larger overlap onto $\etaSinglet \omegaSinglet$ operators shown in cyan.
}
\label{1m_coupled}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

These $t$-matrices have pole singularities on sheets ${\mathsf{III}( \mathrm{Im}\, k_{\etaOctet \omegaOctet} \!<\! 0, \mathrm{Im}\, k_{\etaSinglet \omegaSinglet} \!<\! 0)}$ and ${ \mathsf{II}( \mathrm{Im}\, k_{\etaOctet \omegaOctet} \!<\! 0, \mathrm{Im}\, k_{\etaSinglet \omegaSinglet} \!>\! 0) }$ that are qualitatively unchanged compared to the elastic-only assumption, albeit with larger statistical uncertainties. While it is not well determined, it is possible that the $\mathsf{b}$--pole may have a modest $\etaSinglet \omegaSinglet$ coupling, $ a_t |c_{\etaSinglet \omegaSinglet} | \lesssim 0.04$, that does not change the total width of the heavier resonance because there is so little phase-space for the decay.


Scattering of $\etaSinglet \omegaSinglet$ in $P$--wave can also impact ${J^{PC} = 2^{--}}$, with the $F$--wave being unlikely to contribute significantly so close to threshold. We augment the pole plus constant $K$-matrix of Eqn.~\ref{J2_pole_const} with an extra $\etaSinglet \omegaSinglet \{ \threePtwo \}$ channel, letting the pole coupling to this new channel and the extra diagonal constant float freely in a description of 96 energy levels, 7 of which have large $\etaSinglet \omegaSinglet$ overlap. The quality of fit, $\chi^2 / N_\mathrm{dof} = \tfrac{125.7}{96 - 9} = 1.45$, is reasonable, and the resulting $t$-matrix elements are shown in Figure~\ref{2m_coupled}. Clearly the additional channel has only a weak effect. The $t$-matrix has a pole (on sheets $\mathsf{III}$ and $\mathsf{II}$) that is in a location compatible with previous estimates. Similarly the $\etaOctet \omegaOctet$ couplings in $P$-- and $F$--waves are not significantly changed. There is a pole coupling to $\etaSinglet \omegaSinglet$ that while small, $a_t | c_{\etaSinglet \omegaSinglet}| \sim 0.07(2)$, is of a comparable size to the $\etaOctet \omegaOctet$ $F$--wave coupling.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 2m coupled  %%
\begin{figure}
%
\includegraphics[width=0.98\columnwidth]{figures/2m_coupled_polish}
%
\caption{$J^{PC} = 2^{--}$ $t$-matrix, as in Figure~\ref{2m3m_ref_rhotsq} (grey), with the addition of the $\etaSinglet \omegaSinglet \{ \threePtwo \}$ channel.
}
\label{2m_coupled}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



It proves to be the case that the large statistical uncertainties on the $\omegaSinglet \fZeroSinglet$ energy levels prevent any meaningful attempt at coupled-channel $(\etaOctet \omegaOctet, \omegaSinglet\! \fZeroSinglet)$ analysis. As such while we cannot rule out non-zero couplings to $\omegaSinglet \fZeroSinglet$ for our resonances, such an outcome seems unlikely given our ability to describe the a huge number of finite-volume energy levels using a set of decoupled amplitudes.


%\color{red}
%We have made efforts to couple the $\omegaSinglet \fZeroSinglet$ to the system in the $1^{--}$, but the statistical uncertainties on these levels are much too large. Matching the finite volume spectrum to the solutions predicted by the quantization condition is no trivial task, and already require relatively good initial guesses for parameterizations. We make use heavily of matching levels with large $\left|\frac{\sigma}{E_{lat}-E_{sol}}\right|^2$, and if $\sigma$ is too large one can imagine nearby solutions produced by levels with little or no $\omegaSinglet \fZeroSinglet$ overlap matching to a one of these noisy levels, producing misleading results.
%\color{black}



%... summarize that there isn't any evidence for significant channel coupling ...
%
%\color{red}
%We see no strong evidence of additional channel coupling through out this analysis. When we relax our decoupled assumption for the $\etaSinglet\omegaSinglet$ channel we find small couplings to the $\etaSinglet\omegaSinglet$ relative to the $\etaOctet\omegaOctet$, and very modest changes (if any) to the pole positions and couplings to $\etaOctet\omegaOctet$ indicating that performing an elastic analysis on $\etaOctet\omegaOctet$ is a perfectly valid approximation. As for the $\omegaSinglet \fZeroSinglet$ channel it can be clearly seen in the finite volume spectrum these levels generally intersect with their corresponding noninteracting energy curves across multiple volumes and \textit{irreps}, heavily indicating this channel is compatible with no scattering at all. We could not quite relax the decoupled assumption for the $\omegaSinglet \fZeroSinglet$ channel in our analysis, but we stress that likely nothing would be gained from doing so. 
%\color{black}



